UIBert: Learning Generic Multimodal Representations for UI Understanding

To improve the accessibility of smart devices and to simplify their usage, building models which understand user interfaces (UIs) and assist users to complete their tasks is critical. However, unique challenges are proposed by UI-specific characteristics, such as how to effectively leverage multimodal UI features that involve image, text, and structural metadata and how to achieve good performance when high-quality labeled data is unavailable. To address such challenges we introduce UIBert, a transformer-based joint image-text model trained through novel pre-training tasks on large-scale unlabeled UI data to learn generic feature representations for a UI and its components. Our key intuition is that the heterogeneous features in a UI are self-aligned, i.e., the image and text features of UI components, are predictive of each other. We propose five pretraining tasks utilizing this self-alignment among different features of a UI component and across various components in the same UI. We evaluate our method on nine real-world downstream UI tasks where UIBert outperforms strong multimodal baselines by up to 9.26% accuracy.

==> dataset.tex <==
\vspace{-1mm}
\section{Downstream tasks and data}\label{sec:data}
\vspace{-1mm}
In this section, we present the downstream tasks to evaluate the pretrained \uibert\ and their datasets.
% \paragraph{Pre-training Data} We obtain 537k pairs of UI screenshots and their view hierarchies using Firebase Robo app crawler\footnote{\url{https://firebase.google.com/docs/test-lab/android/robo-ux-test}}. 
%In each batch of pre-training, a fake UI is generated on-the-fly from each original UI (example in Fig. \ref{fig:fake_ui}). 
% Our model is pre-trained on the large-scale dataset without any human annotation.
%\paragraph{Rico Data} Rico \cite{Deka2017Rico} is a public mobile design dataset containing 72k unique UI screenshots with view hierarchies crawled across 9.7k mobile apps. We establish five downstream tasks based on it as described below.
%Below we describe five kinds of downstream tasks that we establish based on it.

\paragraph{Similar UI component retrieval.} Given an anchor UI with an anchor component as the query and a seacrh UI with a set of candidate components, the task selects the closest candidate to the anchor component in terms of functionality (Fig.~\ref{fig:task-vis}(a)). One dataset for this task is extended from Rico \cite{Deka2017Rico}, a public mobile design dataset containing 72k unique UI screenshots with view hierarchies crawled across 9.7k mobile apps. It consists of 1M anchor-search UI component pairs annotated via a combination of crowd-sourcing and programmatic rules%(Appendix)
: 900k for training and 32k respectively for dev and test. 
On average, each search UI has 10 candidate components for the model to choose from. 
The dataset will be released upon paper publication. 
Another dataset for this task includes 65k anchor-search web UI pairs. Each search web UI has 35 components on average. 
Note that as view hierarchies are unavailable in web UIs, there is no VH inputs to \uibert\ during finetuning.
%We curate from Rico 900k anchor-search UI pairs with anchor and candidate components annotated via crowd-sourcing. On average, each search UI has 10 candidate components. The dataset will be released upon paper publication. 

\paragraph{Referring expression component retrieval.} Given a referring expression and a UI image, the goal is to retrieve the component that the expression refers to from a set of UI components detected on the screen (Fig. \ref{fig:task-vis}(b)). This task has a practical use for voice-control systems. UIs of this task are selected from Rico and the referring expressions are collected by crowdsourcing. 
On average, each expression has 20 UI component candidates on the given UI.
% the model needs to choose from 20 UI components on the given UI for every expression. 
The train, dev, and test sets respectively contain 16.9k, 2.1k and 1.8k UI componenets with their referring expressions. 
%The dataset for this task contains 16.9k pairs of referring expressions and UIs that have a list of UI components that are selected from , where 20 components are available per UI on average. The data will also be released. 

\paragraph{Image-VH sync prediction.} View hierarchies can be noisy when unsynchronized with screenshots (\cite{li2020mapping}). This task takes the UI screen with its VH as input and outputs whether the VH matches the screen. It can serve as an important pre-processing step to filter out the problematic UIs. We use the RicoSCA (\cite{li2020mapping}) that have 25k synchronized and 47k unsynchronized UIs and split them into train, dev, and test sets by a ratio of 8:1:1.

\paragraph{App type classification.} This task aims to predict the type of an app (e.g. music, finance) of a UI. We use all the 72k unique UIs in Rico across a total of 27 app types and split them in the ratio of 8:1:1 for train, dev, and test.  %Overall, there are 27 app types from 72k Rico UIs extracted in Google Play. 
%Since the app type is required by Google Play, 
This task can help filter the malicious apps that have incorrect app types.
% The model trained for this task can help to filter the malicious apps that have incorrect app types.

\paragraph{Icon classification.} This task aims to identify the types of icons (e.g. menu, backward, search). As icons are common components, their types provide important information which can be used by screen readers. We use the human-annotated icon labels from \cite{he2021ab} on Rico data in two levels of granularity: 32 and 77 classes. 
The icons are labeled on view hierarchy leaf nodes of each UI 
% , and each UI may have multiple icons. 
In total, there are 644,931 and 601,878 labels for 32 and 77 classes respectively.

% \paragraph{Web Data} To conduct the similar UI component retrieval task in websites, we use the dataset collected by \cite{he2021ab} including 65k anchor-candidate web UI screen pairs (35 components avg. per candidate UI). Note view hierarchies are unavailable in this data. 

% On all the datasets, we extract the OCR texts associated with bounding boxes using the MLKit API\footnote{https://developers.google.com/ml-kit/vision/text-recognition/android}.

\begin{figure}
\includegraphics[width=\columnwidth]{figs/vis-example.png}
\centering
\vspace{-5mm}
\caption{a) An example of similar UI component retrieval. b) An example of referring expression component retrieval.}\label{fig:task-vis}
\vspace{-5mm}
\end{figure}
%task where one is required the semantically similar UI Component from search UI to the anchor UI component in anchor UI

==> experiment.tex <==
\vspace{-1mm}
\section{Experiments}
\vspace{-1mm}
% \subsection{Pretraining}
% \vspace{-1mm}


\subsection{Quantitative Evaluation}\label{sec:exp-finetune}
\vspace{-1mm}
We evaluate the pretrained \uibert\ on nine practical downstream tasks across five categories, including two zero-shot tasks. During fine-tuning, \uibert\ is trained for 200k steps with dropout rate of 0.1, using the same optimizer configuration and batch size as pretraining.

\paragraph{Baselines} We consider two baseline encoding mechanisms for the downstream tasks: \emph{EfficientNet+Albert} and \emph{ActionBert}. The first one uses EfficientNet-B0  and Albert \cite{lan2019albert} to encode the image and text components of the UI separately. As there is no attention across the two modalities, it serves as an ablation evaluation for the Transformer blocks used in \uibert\ which facilitate this cross-modal attention. The second baseline, ActionBert \cite{he2021ab}\footnote{We use ActionBert$_{BASE}$ due to its comparable size to \uibert.}, is a recently proposed UI representation model, pretrained with user interaction traces. 

For prediction, the embedding of each image component is the concatenation of content embeddings from the OBJ and its aligned VH component, and the UI-level embedding is the max pooling of all content embeddings.
% For component-level tasks, the embeddings of each OBJ and its aligned VH component are concatenated. For UI-level tasks, the max pooling of all embeddings are used.
All results are obtained from the same training and test splits.

\paragraph{Similar UI Component Retrieval} We conduct this task on both the Rico and Web data described in Sec.\ref{sec:data}. The anchor UI and search UI are fed into \uibert\ separately to get the output embeddings, then the dot products between embeddings of anchor component and candidate components are used as similarity scores to predict the most similar candidate to the anchor. We finetune \uibert\ using the multi-class cross entropy loss on the similarity scores. Since no additional model parameters are needed, the task is also evaluated in a zero-shot manner by directly using the pretrained model. \emph{Since web data has no view hierarchy, the input view hierarchy components are empty in \uibert}.

Overall, prediction accuracy of all methods on the four task variations are reported in Tab. \ref{tab:sim-retri}. We observe that \uibert\ outperforms both baselines on all cases by 1.58\%--14.16\%, especially by a large margin on the zero-shot tasks, showing the advantages of our pretraining techniques. 

\begin{table}[]
    \centering
    \resizebox{0.65\columnwidth}{!}{
    \begin{tabular}{lcccc}
    \toprule
     & \multicolumn{2}{c}{Fine-tune} & \multicolumn{2}{c}{Zero-shot} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
    Model & Rico data & Web data & Rico data & Web data \\
    \midrule
    EfficientNet+Albert & 85.70 & 62.11 & 22.18 & 18.80 \\
    ActionBert & 85.38 & 62.85 & 30.42 & 24.80  \\
    \uibert\ & \textbf{88.18} & \textbf{65.31} & \textbf{38.00} & \textbf{32.82}  \\
    \bottomrule
    \end{tabular}
    }
    \vspace{-2mm}
    \caption{Prediction accuracy (\%) on 4 similar UI component retrieval tasks. On average, the model chooses one from 10 and 35 candidates on Rico and Web data respectively. \label{tab:sim-retri}}
\end{table}
% \begin{table}[]
%     \centering
%     \resizebox{0.35\columnwidth}{!}{
%     \begin{tabular}{lc}
%     \toprule
%     EfficientNet+Albert & 86.98  \\
%     ActionBert & 88.38 \\
%     \uibert\ & \textbf{91.84} \\
%     \bottomrule
%     \end{tabular}
%     }
%     \caption{Prediction accuracy (\%) on the referring component retrieval task. The model needs to retrieve 1 from 20 candidates avg. \label{tab:vis}}
% \end{table}

% \begin{table}[h]
%     \centering
%     \resizebox{0.6\columnwidth}{!}{
%     \begin{tabular}{lcc}
%     \toprule
%     & Accuracy (\%) & Macro-F1\\
%     \midrule
%     EfficientNet+Albert & 77.58 & 0.7500  \\
%     \uibert\ & \textbf{78.93} & \textbf{0.7704} \\
%     \bottomrule
%     \end{tabular}
%     }
%     \caption{Prediction results on the image-VH sync prediction task. \label{tab:img-vh-sync}}
% \end{table}

% \begin{table}[h]
%     \centering
%     \resizebox{0.9\columnwidth}{!}{
%     \begin{tabular}{lcc}
%     \toprule
%     & Acc. (\%) & Macro-F1 \\
%     \midrule
%     EfficientNet+Albert & 66.35 & 0.6307 \\
%     ActionBert\footnote{The results are different from that reported in \cite{he2021ab}, which only used a subset (43.5k out of 72k) of Rico data.}  & 72.60 & 0.6989 \\
%     \uibert\ & \textbf{72.69} & \textbf{0.6998} \
%     \bottomrule
%     \end{tabular}
%     }
%     \caption{Prediction results on app type classification. \label{tab:app-type}}
% \end{table}

\begin{table}[h]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{lcc|cc|c}
    \toprule
    & \multicolumn{2}{c}{image-VH sync prediction} & \multicolumn{2}{c}{App type classification}  & Ref. expression comp. retrieval\\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-6}
    Model & Acc. (\%) & Macro-F1 & Acc. (\%) & Macro-F1 & Acc. (\%) \\
    \midrule
    EfficientNet+Albert & 66.35 & 0.6307 & 77.58 & 0.7500 & 86.98\\
    ActionBert\footnote{The results are different from that reported in \cite{he2021ab}, which only used a subset (43.5k out of 72k) of Rico data.}  & 72.60 & 0.6989 & - & - & 88.38\\
    \uibert\ & \textbf{72.69} & \textbf{0.6998} & \textbf{78.93} & \textbf{0.7704} & \textbf{91.84}\\
    \bottomrule
    \end{tabular}
    }
    \vspace{-2mm}
    \caption{Prediction results on three downstream tasks: image-VH sync prediction, app type classification, and referral expression component retrieval.\label{tab:result-sync-vis-app}}
\end{table}


\begin{table}[]
    \centering
    \resizebox{0.7\columnwidth}{!}{
    \begin{tabular}{lcccc}
    \toprule
     & \multicolumn{2}{c}{Icon-32} & \multicolumn{2}{c}{Icon-77} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} 
    Model & Acc. (\%) & Macro-F1 & Acc. (\%) & Macro-F1 \\
    \midrule
    EfficientNet+Albert & 97.42 & 0.8723 & 92.29 & 0.6549 \\
    ActionBert & 97.42 & 0.8742 & 91.60 & 0.6376  \\
    \uibert\ & \textbf{97.56} & \textbf{0.8788} & \textbf{92.50} & \textbf{0.6621}  \\
    \bottomrule
    \end{tabular}
    }
    \vspace{-2mm}
    \caption{Prediction results on two icon classification tasks. \label{tab:icon-cls}}
\end{table}

\paragraph{Referring Expression Component Retrieval} As inputs in addition to the UI components, the referring expression is treated as an OCR component while the candidates are added to the OBJ components. Like the similar UI component retrieval task, dot products between the output embedding of the referring expression and output embeddings of candidates are computed as similarity scores to select the referred component. The prediction results can be found in Tab. \ref{tab:result-sync-vis-app}. \uibert\ achieves the best accuracy 91.84\%, which clearly outperforms ActionBert by 3.46\%. 
% All models are fine-tuned using the multi-class cross entropy loss.

\paragraph{Image-VH Sync Prediction} The output embedding of the CLS component is connected with a one-layer MLP to predict whether the image and view hierarchy of an UI are synced. Tab. \ref{tab:result-sync-vis-app} shows that \uibert\ achieves 78.93\% accuracy and 77.04\% macro-F1, which outperform the baseline by 1.36\% and 1.79\% respectively.

\paragraph{App Type Classification} To predict one of the 27 app types given an UI, we expect a prediction head to summarize all UI components. Thus, concatenation of all component UI embeddings are fed into a one-layer MLP. As shown in Tab. \ref{tab:result-sync-vis-app}, \uibert\ largely outperforms the EfficientNet+Albert baseline by 6.34\% accuracy and 6.91\% Macro-F1, showing the gain from fusing components via the transformer block and from pretraining. Moreover, \uibert\ slightly outperforms ActionBert by ~0.1\% accuracy and F1.

\paragraph{Icon Classification} To predict the types of an icon component, we concatenate the UI embeddings of the icon's corresponding OBJ and VH components and feed into a one-layer MLP. Tab. \ref{tab:icon-cls} shows the prediction results on both 32 and 77 classes granularity. \uibert\ consistently outperforms baselines by 0.14--0.9\% accuracy and by 0.46--2.45\% F1, with a larger gain on the icon-77 task.








%=============================
% For 32 classes (icon-32), \uibert\ is better than baselines by 0.14\% accuracy and 0.46\%--0.65\% Macro-F1. For 77 classes, although the overall performance drops, \uibert\ outperforms baselines by a larger margin: 0.21\%--0.9\% accuracy and 0.72\%--2.45\% Macro-F1.

%-------------------------
% Qualitative evaluation
% \begin{figure}
% \centering
%   \includegraphics[width=\linewidth]{figs/embedding_tsne.png}
% \vspace{-5mm}
% \caption{Embedding visualization for top-5 common app and icon types using T-SNE. No fine-tuning is needed. Best viewed in color.\label{fig:emb_tsne}}
% \end{figure}

% \begin{figure}
% \centering
% \begin{subfigure}{.48\columnwidth}
%   \centering
%   \includegraphics[width=\linewidth]{figs/app5_tsne}
%   \caption{Top-5 app types (1921 points).}
%   \label{fig:app_tsne}
% \end{subfigure}%
% \begin{subfigure}{.48\columnwidth}
%   \centering
%   \includegraphics[width=\linewidth]{figs/icon5_tsne}
%   \caption{Top-5 icon types (5169 points). }
%   \label{fig:icon_tsne}
% \end{subfigure}
% \caption{Embedding visualization for top-5 common app and icon types using T-SNE. No fine-tuning is needed. Best viewed in color.}
% \end{figure}

% \subsection{Qualitative Evaluation}\label{sec:quality_eval}
% \vspace{-1mm}
% To demonstrate the quality of \uibert\, without any fine-tuning, we visualize the pretrained UI-level and component-level embeddings, and showcase generating content descriptions.
% % We also visualize the UI embeddings and the generated content descriptions from \uibert. 
% \paragraph{Embedding Visualization} 
% We use t-SNE \cite{maaten2008visualizing} to visualize the embeddings from the pretrained \uibert.  Fig. \ref{fig:emb_tsne} shows the 2D visualizations of embeddings associated with top-5 common app types and icon types respectively. We observe that even \emph{without} fine-tuning, the embeddings are grouped together by app types and icon types respectively, which suggest that \uibert\ captures the semantics of app types and icon types. 

% \paragraph{Content Description Generation}
% Note that generating content descriptions of view hierarchy nodes based on contextual information is one of the pretraining tasks (MVG) for \uibert.
% %As pretrained with the MVG task, \uibert\ can generate content descriptions of view hierarchy nodes based on its contextual information.
% We mask all the content descriptions in the test set of Image-VH sync prediction task, and generate them using
% %the pretrained 
% \uibert\ without any fine-tuning. As shown in Fig. \ref{fig:content_desp},
% most of the generated descriptions are correct. Some are incorrect but reasonable (case 5).
%We notice that the model generates correct descriptions in most cases and sometimes reasonable yet incorrect predictions (case 5), which indicates the efficacy of the MVG pretraining task.
%the correct descriptions are generated and the  in some cases (4,5,10) they are partially correct, and totally wrong. \emph{In the whole data, 70\% of generated descriptions are exactly correct.} This indicates the efficacy of the MVG pre-training task.
% \begin{figure}[ht]
% \centering
% \includegraphics[width=\linewidth]{figs/content_desp.png}
% \vspace{-5mm}
% \caption{Examples of generated content descriptions by a pretrained \uibert\ (correct in blue and incorrect in red).\label{fig:content_desp}}
% \end{figure}

% \begin{table}[]
%     \centering
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{l|ccccc|c}
%     \toprule
%      & \multicolumn{5}{c}{Pre-training Tasks}\\
%     \cmidrule(lr){2-7}
%     Downstream Tasks & -- & Mask-freeze & Mask & Mask,RUI & Mask,RCP & All \\
%     \midrule
%     Similar UI Comp. Retri.-Rico & 87.95 & 87.82 & 87.80 & 88.11 & 88.13 & \textbf{88.18} \\
%     Similar UI Comp. Retri.-Web & 64.58 & 58.59 & 64.84 & 65.05 & \textbf{65.73} & 65.31 \\
%     Ref. Expression Comp. Retri. & 88.54 & 90.42 & 90.80 & 91.35 & 90.93 & \textbf{91.84} \\
%     Image-VH Sync Prediction & 77.34 & 78.47 & 75.97 & 77.47 & 77.77 & \textbf{78.93} \\
%     App Type Classification & 68.16 & 68.20 & 69.41 & 70.32 & 69.43 & \textbf{71.32} \\
%     Icon-32 Classification & 97.43 & 97.50 & 97.44 & 97.47 & 97.44 & \textbf{97.56} \\ 
%     Icon-77 Classification & 92.12 & 92.10 & 91.86 & 92.06 & 91.99 & \textbf{92.50} \\ 
%     \bottomrule
%     \end{tabular}
%     }
% \vspace{-2mm}
% \caption{Ablation study for different pre-training tasks. Accuracy on downstream tasks is reported. ``Mask'' stands for the three masked component prediction tasks: MIP, MOG and MVG. ``Mask-freeze'' means that during pre-training, the image and text encoders are frozen like ActionBert.\label{tab:ablation}}
% \end{table}
% \subsection{Ablation Study}
% \vspace{-1mm}
% In this experiment, we conduct ablation study to analyze the effects of different pre-training tasks. Tab. \ref{tab:ablation} shows the accuracy of fine-tuning the model on all downstream tasks using different combinations of the pre-training tasks. ``-'' means no pre-training (train the model from scratch), ``Mask'' denotes the combination of three masked component prediction tasks (MIP, MOG, MVG), and ``Mask-freeze'' means freezing the image and text encoders during pre-training. 

% Overall, we observe that \uibert\ with \emph{all} pre-training tasks achieves the best performance except for the web similar UI component retrieval task, in which pre-training with Mask and RCP tasks achieves the best accuracy. Moreover, training from scratch (second column) performs worse than using pre-training (last column) across all the downstream tasks, indicating the effectiveness of our proposing pretraining tasks.

%beating \uibert\ with all tasks pre-trained by 0.42\%
